Mitigating Noisy Correspondence by Geometrical Structure Consistency Learning

Noisy correspondence that refers to mismatches in cross-modal data pairs, is prevalent on human-annotated or web-crawled datasets. Prior approaches to leverage such data mainly consider the application of uni-modal noisy label learning without amending the impact on both cross-modal and intra-modal geometrical structures in multimodal learning. Actually, we find that both structures are effective to discriminate noisy correspondence through structural differences when being well-established. Inspired by this observation, we introduce a Geometrical Structure Consistency (GSC) method to infer the true correspondence. Specifically, GSC ensures the preservation of geometrical structures within and between modalities, allowing for the accurate discrimination of noisy samples based on structural differences. Utilizing these inferred true correspondence labels, GSC refines the learning of geometrical structures by filtering out the noisy samples. Experiments across four cross-modal datasets confirm that GSC effectively identifies noisy samples and significantly outperforms the current leading methods.

==> sec/1_intro_1117.tex <==
\section{Introduction}
\label{Section: Introduction}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.47\textwidth]{pics/introduction.png}
% [width=1.30\textwidth]
\caption{Illustration of noisy correspondence with its effects. A puppy is mistaken to be annotated with a kitten in the noisy correspondence example in the middle, which is common in real-world datasets and can cause damage to both cross-modal and intra-modal geometrical structures.}
\label{Figure: Introduction}
\end{center}
\end{figure}

Cross-modal retrieval, which focuses on retrieving the most relevant samples across different modalities, has garnered considerable interest as a key task in multimodal scenarios~\cite{malinowski2015ask, vinyals2015show, xu2015show, chen2023enhanced, diao2021similarity}. Most current retrieval models presuppose that a large quantity of well-annotated data is available. However, real-world datasets, often resort to non-expert annotation or web crawling due to time and budget constraints, are prone to noisy correspondence~\cite{sharma2018conceptual, jia2021scaling, chua2009nus, chen2023redundancy}. Noisy correspondence refers to the mismatches between modalities in collected data pairs. Such discrepancy can cause severe degradation to retrieval models if without proper handling~\cite{huang2021learning}.

Recently, the challenge of learning with noisy correspondence has gathered increasing attention from researchers. The majority of these efforts share a common target of accurately learning soft correspondence labels that can reliably indicate the matching degree between data pairs. To be specific, NCR~\citep{huang2021learning} pioneered this area by employing a co-teaching approach to classify samples with higher losses as noisy. Such method, which has been further refined by \citet{yang2023bicro, han2023noisy} by introducing meta-learning and leveraging clean data subsets, however fundamentally remains a variation of the uni-modal sample selection method~\citep{li2020dividemix}, which may not fully address the intricacies of multimodal learning. While other works aim to enhance the robustness of retrieval models through robust loss functions, they fail to further improve the performance without explicitly excluding the noisy samples. %最后面这一类加引用，加粗线条

Distinct from the noisy label problem in uni-modal learning, noisy correspondence affects the geometrical structures of multimodal representations from both cross-modal and intra-modal aspects. Consider the contrastive learning optimization process, as depicted in Figure~\ref{Figure: Introduction}, the paired text acts as a positive key to the query image, contrasting with negative keys from other texts. If the paired data is noisy, the cross-modal distance between the query and its positive key is erroneously reduced. Concurrently, the query image is drawn closer to a cluster of images that resemble the text of the noisy positive key. Despite these challenges, we have observed significant differences between clean and noisy samples within well-established cross-modal and intra-modal geometrical structures (as detailed in Section~\ref{Section: Motivation}). These differences offer a promising strategy for discriminating noisy samples and accurately predicting true correspondence labels.

Building on this concept, we introduce the Geometrical Structure Consistency (GSC) method to mitigate the issue of noisy correspondence. GSC maintains the integrity of geometrical structures by adding a contrastive loss that aligns the intra-modal geometrical structures along with the traditional loss for cross-modal alignment. Benefiting from the memorization effect of DNNs~\cite{xia2020robust, arpit2017closer}, geometrical structure can be well-established in the early stage. During this phase, GSC assesses the true soft correspondence labels based on the differences in geometrical structure within and across modalities. For the cross-modal aspect, GSC identifies potential noise by recognizing data pairs with low cross-modal similarities, while in the case of intra-modal aspect, the similarity between the queried sample and other samples are calculated to determine the intra-modal geometrical structure, and data pairs with inconsistent structures across modalities are considered as noisy. These assessed labels are then used to clarify the learning of the geometrical structure, creating a positive feedback loop. To conclude, the contributions of this work are summarized as follows:
\begin{itemize}
    \item We acknowledge the unique complexities of multimodal scenarios, being aware of the detrimental effects of noisy correspondence on both cross-modal and intra-modal geometrical structures. 
    \item We introduce the innovative Geometrical Structure Consistency (GSC) approach, which leverages differences in geometrical structure to accurately identify true correspondence labels and counteract the adverse effects of noisy correspondences.
    \item Our proposed GSC method is not only novel but also compatible with existing approaches for handling noisy correspondences. Through extensive testing on three benchmark datasets, we have proven the consistent efficacy of our method.
\end{itemize}

==> sec/2_relatedwork_1117.tex <==
\section{Related Works}
\label{Section: Related Works}

\subsection{Cross-modal Retrieval}
Cross-modal retrieval focuses on using one modality information as a query to search for and retrieve related data in other modalities~\citep{liu2022regularizing, huang2022mack, goel2022cyclip, pan2023fine, fu2023learning}. Due to the restriction of large-scale annotated multi-modal corpus, the unsupervised guided framework has always been the mainstream.
VSE++~\citep{faghri2017vse++} strategically utilized hard negatives to boost its retrieval efficacy based on hard negative mining. SCAN~\citep{lee2018stacked} implemented a stacked cross-attention framework, allowing for dual-context attention involving both images and sentences to dissect the nuanced interplay between modalities. SGRAF~\citep{diao2021similarity} harnessed Graph Neural Network to achieve granular correspondences and an attention mechanism to select the most representative alignments, thereby enhancing the precision of cross-modal similarity assessments.


However, these cross-modal retrieval methods highly rely on well-aligned data while neglecting the existence of noisy correspondence within the dataset, which may inevitably degrade the vanilla model performance.

\subsection{Noisy Correspondence Learning}
% NCR DECL BICRO MSCN
Noisy correspondence was first aroused in~\citep{huang2021learning}, which is a novel paradigm in the field of noise learning, referring to the mismatched pairs within the multi-modal dataset. To tackle this problem, NCR~\citep{huang2021learning} utilized the introduced DivideMix architecture to distinguish clean pairs from noisy ones and rectify the noisy correspondence based on the memorization effect of DNNs. \citet{yang2023bicro} further improved NCR by switching Gaussian Mixture Model to Beta Mixture Model and integrated a new soft correspondence label estimation method. \citet{qin2022deep} combined the idea of evidential learning with noisy correspondence and put forward a confidence-based method, achieving better retrieval performance under extreme noise rates and alleviating computation costs. \citet{han2023noisy} proposed a meta-similarity correction network that reinterprets binary classification of correct and noisy correspondences as a meta-process, enhancing data purification. Although these models have showcased promising performances, they only cast their spotlight on interactions across modalities, which is insufficient in utilizing the semantic-abundant cross-modal data, further motivating us to take not only inter-modal but also intra-modal together into consideration to help mitigate noisy correspondence.


==> sec/3_method_1112.tex <==
\section{Proposed Method}
\label{Section: Method}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\textwidth]{pics/structure.png}
% [width=1.30\textwidth]
\caption{An overview of CDL. \textbf{Left:} The framework of CDL, benefiting from the concluded relationships, CDL re-weights typical correspondence learning loss to explain away noisy correspondence. \textbf{Right:} CDL assigns lower weights on noisy samples. Specifically, the weight relies on the matrix producted by two logits to estimate the coupling and decoupling terms. The coupling term concerns the diagonal elements of the matrix while the decoupling term concerns the non-diagonal ones.}
\label{Figure: Structure}
\end{center}
\end{figure*}

\subsection{Preliminary}

We start by defining notations for cross-modal retrieval in the presence of noisy correspondences, employing the widely studied image-text retrieval task as a generalized exemplar. Consider a multimodal dataset $\mathcal{D} = \{I_i, T_i, y_i\}_{i=1}^N$, where $I_i, T_i$ is the $i$-th image-text pair and the associated label $y_i$ indicates whether the pair is positively correlated ($y_i=1$) or not ($y_i=0$). Note that these labels may contain noise, as pairs in the dataset are often presumed to be matched. Typical cross-modal retrieval models include separate encoders for image and text modalities as $f$ and $g$, and a similarity module $S$ calculating the similarity scores between extracted representations as $S(X, Y)$, or shortened as $\langle X, Y\rangle$.

% We start by formulizing the task of cross-modal retrieval within the context of noisy correspondences. We use the commonly studied image-text retrieval task as an example, which broadly represents the challenges without compromising generality. Consider a cross-modal dataset $\mathcal{D} = \{I_i, T_i, y_i\}_{i=1}^N$, where $I_i, T_i$ is the $i$-th image-text pair and the associated label $y_i$ indicates whether the pair is positively correlated ($y_i=1$) or not ($y_i=0$). Note that these labels may contain noise, as pairs in the dataset are often presumed to be matched. Denote the separate encoders for image and text modalities as $f$ and $g$, typical cross-modal retrieval models calculate the similarity score $S(f(I), g(T))$ (shortened to $\big<I,T\big>$) and optimize the following contrastive loss to reach cross-modal alignment.
% \begin{equation}
% \begin{aligned}
%  \mathcal{L}_{\text{CM}} =& -\frac{1}{2N}\sum_{i=1}^N\log{\frac{\exp{(\big<I_i, T_i\big>/\tau_1)}}{\sum_{j=1}^N\exp{(\big<I_i, T_j\big>/\tau_1)}}} \\
%  & -\frac{1}{2N}\sum_{j=1}^N\log{\frac{\exp{(\big<I_j, T_j\big>/\tau_1)}}{\sum_{i=1}^N\exp{(\big<I_i, T_j\big>/\tau_1)}}}
% \label{Equal: Cross-modal Loss}
% \end{aligned}
% \end{equation}

% \noindent
% in which $\tau_1$ is the temperature coefficient. The former part contrasts the query image with key texts and the latter part contrasts the query text with key images.

\subsection{Motivation}
\label{Subsection: Motivation}

The contrastive loss in Eq.~\ref{Equal: Cross-modal Loss} directly closen the distance between modalities without maintaining intra-modal structure, is argued to be sub-optimal for inconsistent reasoning~\citep{goel2022cyclip, jiang2023understanding}. Thus we propose an additional regularization with contrastive loss to preserve the consistency of 
intra-modal geometrical structure among modalities.
\begin{equation}
 \mathcal{L}_{\text{IM}} = -\frac{1}{N}\sum_{i=1}^N\log{\frac{\exp({\sum_{k=1}^N\big<I_i,I_k\big>\big<T_i,T_k\big>/\tau_2)}}{\sum_{j=1}^N\exp{(\sum_{k=1}^N\big<I_i, I_k\big>\big<T_j, T_k\big>/\tau_2)}}}
\label{Equal: Intra-modal Loss}
\end{equation}

\noindent
in which $\tau_2$ is also a temperature coefficient. GSC optimizes the $\gamma$-weighted combination of two losses as Eq.~\ref{Equal: Overall Loss} to establish stable cross-modal and intra-modal structures. However, both structures can be affected by noisy correspondences in different manners, which can be observed in the subsequent experimental phenomena.
\begin{equation}
 \mathcal{L} = \mathcal{L}_{\text{CM}} + \gamma\mathcal{L}_{\text{IM}}
\label{Equal: Overall Loss}
\end{equation}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.47\textwidth]{pics/motivation.png}
% [width=1.30\textwidth]
\caption{The impact of noisy correspondence on both cross-modal and intra-modal structures. Left: Curve of $\mathcal{L}_{\text{CM}}$ on train set and test set. Right: Curve of $\mathcal{L}_{\text{IM}}$ on train set and test set. These experiments were conducted on the Flickr30K dataset with 40\% noise. The test set curve is interpolated and smoothed as the loss is computed at each epoch.}
\label{Figure: Motivation}
\end{center}
\end{figure}

As illustrated in Figure~\ref{Figure: Motivation}, the plain cross-modal retrieval model is optimized by Eq.~\ref{Equal: Overall Loss} without incorporating denoising techniques. For the cross-modal aspect, noisy correspondence can align the mismatched representations among modalities, leading to increasing similarity scores of noisy samples as the training process converges. For the intra-modal aspect, noisy correspondence affects the structure in two ways. Firstly, the geometrical structure of the query sample is inaccurately calculated by including the distance to noisy samples. Secondly, the alignment of intra-modal structures among noisy samples can also affect the learning process. Since the composition of samples within a batch is constantly changing, the retrieval model ultimately tends to predict an averaged similarity score across all samples, leading to the collapse of the intra-modal structure. 

Despite these challenges, it is important to notice that both cross-modal and intra-modal can form a well-established structure in the initial stages of training, during which clean samples are observed with higher cross-modal similarity scores and more closely aligned intra-modal geometrical structures. Such phenomenon, together with the trend of recall scores on the test set that initially increasing before declining during experiments, indicates the memorization effect of DNNs, which serves as the foundation for our GSC method. In the following sections, we will delve into the details of how GSC leverages these early-stage established structures to effectively discriminate noisy samples.

\subsection{Cross-modal Discrimination}

Assuming a well-established cross-modal structure, clean data pairs are expected to exhibit more closely aligned cross-modal representations compared to noisy pairs. GSC leverages this structural discrepancy and introduces a function to signify the true correspondence indicator.
\begin{equation}
 y_{\text{CM}}^i = \frac{1}{2}\big(\frac{\exp{(\big<I_i, T_i \big>)}}{\sum_{j}^N\exp{(\big<I_i, T_j\big>)}} + \frac{\exp{(\big<I_i, T_i \big>)}}{\sum_{j}^N\exp{(\big<I_j, T_i\big>)}}\big)
\label{Equal: Cross-modal Indicator}
\end{equation}

The indicator measures the proportion of similarity between the query and the positive key against the similarity between the query and other keys. For a clean sample, the similarity between the query and the positive key should dominate the proportion, thus the value of indicator should approach 1. Conversely, for a noisy sample, the similarity between the query and its positive key would be closer to 0, resulting in the indicator's value trending toward 0.

\subsection{Intra-modal Discrimination}

For the intra-modal aspect, the loss function encourages data pairs to exhibit analogous geometrical structures. To illustrate, we compute the similarity vector between a queried image $I_i$ and other images, denoted as $\mathbf{s}_{I_i} =[\big<I_i, I_j\big>]_{j=1}^N$. Similarly, we determine the similarity vector between a queried text $T_i$ and other texts, represented by $\mathbf{s}_{T_i} =[\big<T_i, T_j\big>]_{j=1}^N$. Ideally, matched image-text pairs should have similarity vectors that mirror each other, whereas mismatched pairs would possess distinct similarity vectors, reflecting their divergent positions within a coherent intra-modal structure. Specifically, we employ cosine similarity to measure the resemblance between similarity vectors as follows.
\begin{equation}
 \textbf{s}_{\text{IM}}^i = \frac{\sum_{j=1}^{N} \langle I_i, I_j \rangle \langle T_i, T_j \rangle}{\sqrt{\sum_{j=1}^{N} \langle I_i, I_j \rangle^2} \sqrt{\sum_{j=1}^{N} \langle T_i, T_j \rangle^2}}
 \label{Equal: Cosine Similarity}
\end{equation}

During experiments, the cosine similarity scores of clean samples are observed consistently higher than those of noisy samples, presenting a bimodal distribution of scores across the dataset. This distribution can be accurately modeled using a two-component Gaussian Mixture Model (GMM)~\citep{li2020dividemix}, described by the equation:
\begin{equation}
 p(\textbf{s}_{\text{IM}}) = \sum_{k=1}^K\alpha_k \phi(\textbf{s}_{\text{IM}}|k)
\end{equation}

Specifically, $\alpha_k$ denotes the $k$-th coefficient and $\phi(\textbf{s}_{\text{IM}}|k)$ is the probability density of the $k$-th component. Consequently, we consider the component with higher values, denoted as $k=k_l$, to represent the estimated score distribution of clean samples. The estimated probability that an observed sample belongs to the clean component $k_l$ can be calculated as follows,
\begin{equation}
 y_{\text{IM}}^i = \frac{\alpha_{k_l}\phi(\textbf{s}_{\text{IM}}^i|k_l)}{\sum_{k=1}^K \alpha_k\phi(\textbf{s}_{\text{IM}}^i|k)}
\end{equation}

So far, we have derived the true correspondence labels, $y_{\text{CM}}$ and $y_{\text{IM}}$, by leveraging the structural differences in both cross-modal and intra-modal contexts. Our objective is to optimally utilize these two labels to surmount the respective challenges and to accurately identify all samples with noisy correspondence. Therefore, we define the final correspondence label for each sample as the minimum of the two labels, expressed as:
\begin{equation}
 y^i = \min\{y_{\text{CM}}^i, y_{\text{IM}}^i\}
 \label{Equal: Minimization}
\end{equation}

\subsection{Noise Purification}

We address the issue of noisy correspondence by refining both cross-modal and intra-modal losses, as specified in Eq.~\ref{Equal: Cross-modal Loss} and Eq.~\ref{Equal: Intra-modal Loss}. Since the estimated label is a soft label with values in the range of [0, 1] which can directly reflect the degree of true correspondence, we can seamlessly apply it to the loss functions on a sample-wise basis. The purified cross-modal loss can be denoted as follows,
\begin{equation}
\begin{aligned}
 \mathcal{L}_{\text{CM}} =& -\frac{1}{2N}\sum_{i=1}^Ny^i\log{\frac{\exp{(\big<I_i, T_i\big>/\tau_1)}}{\sum_{j=1}^N\exp{(\big<I_i, T_j\big>/\tau_1)}}} \\
 & -\frac{1}{2N}\sum_{j=1}^Ny^j\log{\frac{\exp{(\big<I_j, T_j\big>/\tau_1)}}{\sum_{i=1}^N\exp{(\big<I_i, T_j\big>/\tau_1)}}}
\label{Equal: Purified Contrastive Loss}
\end{aligned}
\end{equation}

In addition to sample-wise purification for the intra-modal loss, it is crucial to prevent the influence of noisy correspondences from distorting the calculation of the geometrical structure. Specifically, when computing the geometrical structure, the distances from the queried sample to those identified as having noisy correspondences should be excluded. The modified intra-model loss denotes as, 
\begin{equation}
 \mathcal{L}_{\text{IM}} = -\frac{1}{N}\sum_{i=1}^N\log{\frac{\exp({\sum_{k=1}^N{y^k}^2\big<I_i,I_k\big>\big<T_i,T_k\big>/\tau_2)}}{\sum_{j=1}^N\exp{(\sum_{k=1}^N{y^k}^2\big<I_i, I_k\big>\big<T_j, T_k\big>/\tau_2)}}}
\label{Equal: Purified Contrastive Loss}
\end{equation}

Furthermore, noisy correspondences can interfere with the discrimination of noisy samples during the computation of cosine similarity scores in Eq.~\ref{Equal: Cosine Similarity}. Therefore, a similar modification is employed as follows,
\begin{equation}
 \textbf{s}_{\text{IM}}^i = \frac{\sum_{j=1}^{N} {y^j}^2\langle I_i, I_j \rangle \langle T_i, T_j \rangle}{\sqrt{\sum_{j=1}^{N} (y^j\langle I_i, I_j \rangle)^2} \sqrt{\sum_{j=1}^{N} (y^j\langle T_i, T_j \rangle)^2}}
 \label{Equal: Purified Cosine Similarity}
\end{equation}

\subsection{Training Schedule}

To integrate the estimation of true correspondence labels with the enhancement of cross-modal retrieval learning, we adopt the temporal ensembling technique, drawing inspiration from \citet{liu2020earlylearning}, to iteratively update the estimated correspondence labels. Specifically, both $y_{\text{CM}}$ and $y_{\text{IM}}$ are updated through a momentum-based combination of the estimates from the current epoch $t$ and the previous epoch $t-1$, prior to the minimization process outlined in Eq.~\ref{Equal: Minimization}, as shown below, 
\begin{equation}
\begin{aligned}
 y_{\text{CM}}^i[t] &= \beta_1 y_{\text{CM}}^i[t] + (1-\beta_1) y_{\text{CM}}^i[t-1], \\
 y_{\text{IM}}^i[t] &= \beta_1 y_{\text{IM}}^i[t] + (1-\beta_1) y_{\text{IM}}^i[t-1]
 \label{Equal: Momentum Update}
 \end{aligned}
\end{equation}

\noindent
where $\beta_1$ and $\beta_2$ are separate momentum. The estimation of true correspondence labels can be further improved by utilizing two separate neural networks, where the true correspondence labels for each network are computed from the output of the other network. The ablation in Section~\ref{Section: Experiment} shows that two networks can significantly improve the performance. In conclusion, the overall procedure of our Geometrical Structure Consistency (GSC) method is depicted in the pseudo-algorithm~\ref{Algorithm}.

\begin{algorithm}[t]
\caption{Pipeline of learning with our GSC method}
\label{Algorithm}
\begin{algorithmic}[1]
\State Initialize parameters for networks $A$ and $B$.
\For{each epoch $t = 1,2,\ldots,T$}
    \For{network $k = A, B$}
        \For{each minibatch $\mathcal{B}$ from $\mathcal{D}$}
            \State Compute representations for $Net_A$ and $Net_B$: $f_{\theta}(I), g_{\theta'}(T)$
            \State Calculate intra-modal and inter-modal similarity vectors
            \State $Net_A$ estimates $y_{\text{CM}}^B$ and $y_{\text{IM}}^B$ from $Net_B$'s output
            \State $Net_B$ estimates $y_{\text{CM}}^A$ and $y_{\text{IM}}^A$ from $Net_A$'s output
            \State Update both sets of labels using temporal ensembling
            \State Compute cross-modal and intra-modal losses for both networks
            \State Optimize $\theta$ using losses from $Net_B$
            \State Optimize $\theta'$ using losses from $Net_A$
        \EndFor
    \State Update estimated labels $y^i = \min\{y_{\text{CM}}^i, y_{\text{IM}}^i\}$ for both networks
    \EndFor
\EndFor
\State \textbf{end for}
\State Refine both $Net_A$ and $Net_B$ using the final estimated labels
\State \textbf{return} Refined models $Net_A(\theta)$, $Net_B(\theta')$
\end{algorithmic}
\end{algorithm}

==> sec/3_method_1116.tex <==
\section{Proposed Method}
\label{Section: Method}
\subsection{Preliminary}

We start by defining notations for cross-modal retrieval in the presence of noisy correspondences, employing the widely studied image-text retrieval task as a generalized exemplar. Consider a multimodal dataset $\mathcal{D} = \{I_i, T_i, y_i\}_{i=1}^N$, where each $I_i, T_i$ represents the $i$-th image-text pair, standard retrieval models project these data pairs into a shared representation space using separate encoders $f$ for images and $g$ for texts. Then similarity scores between the representations are computed through cosine similarity or an inference model, denoting as $S(f(I), g(T))$, or $\langle I, T \rangle$ in brief. The associated label $y_i$ indicates whether the pair is positively correlated ($y_i=1$) or not ($y_i=0$). Note that these labels may contain noise, as pairs in the dataset are often presumed to be matched. To address this issue, we introduce the \textit{Geometrical Structure Consistency} learning method to identify and correct noisy correspondences, which is detailed in the following sections.

\subsection{Geometrical Structure Consistency Learning}
\label{Section: Motivation}

\noindent
\textbf{Training Objective.} The GSC's training objective encompasses optimizations on both cross-modal and intra-modal structures. From the cross-modal aspect, GSC aims to align the representations among modalities according to the correspondence labels, which is consistent with conventional retrieval models. The expected risk is minimized as shown,
\begin{equation}
\mathcal{R}_{\mathcal{L}_{\text{CM}}}(f, g) = \min_{f, g} \mathbb{E}_{(I, T, y) \sim \mathcal{D}} \left[ \mathcal{L}_{\text{CM}}(\langle I, T\rangle, y) \right]
\label{Equal: Cross-modal Loss}
\end{equation}

\noindent
Here, $\mathcal{L}_{\text{CM}}$ is the cross-modal loss function, typically a contrastive or triplet loss. This function aims to maximize the similarity score $\langle I, T \rangle$ for matching pairs ($y_i=1$). However, optimizing without regard for maintaining intra-modal structure is considered sub-optimal for inconsistent reasoning~\citep{goel2022cyclip, jiang2023understanding}. The intra-modal geometrical structure refers to the relationship between representations within either modality. To uphold the consistency of such structure, GSC incorporates an auxiliary objective as following,
\begin{equation}
 \mathcal{R}_{\mathcal{L}_{\text{IM}}}(f, g) = \min_{f, g} \mathbb{E}_{(I, T, y) \sim \mathcal{D}} \left[ \mathcal{L}_{\text{IM}}(\langle I, I\rangle, \langle T, T \rangle, y) \right]
\label{Equal: Intra-modal Loss}
\end{equation}

\noindent
In this equation, $\mathcal{L}_{\text{IM}}$ denotes the intra-modal loss function. The intra-modal objective ensures that the intra-modal structures of matching samples are constrained to be similar across modalities. GSC simultaneously optimizes both objectives to establish stable cross-modal and intra-modal structures.

\noindent
\textbf{Structural Difference.} Apart from the direct benefits, geometrical structure consistency is instrumental in identifying noisy samples. As depicted in Figure~\ref{Figure: Motivation}, the retrieval model is optimized to converge with both objectives on the clean dataset to form a well-established representation structure, which is then assessed against a dataset with simulated noise. During the experiment, remarkable difference between clean and noisy samples can be observed in both cross-modal and intra-modal structures. Specifically, for cross-modal structure, clean samples typically exhibit higher similarity scores than those noisy ones. Such disparity in distribution originates from the setting that noisy samples are never learnt. For intra-modal structure, the calculated similarities between intra-modal structures of clean and noisy samples manifest a bimodal distribution, suggesting that noisy samples tend to have asymmetric intra-modal structures. Consequently, the training process of GSC evolves into a trilogy: maintaining a stable overall structure, accurately predicting the true correspondence indicator based on structural differences, and mitigating noisy correspondence using this indicator.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.47\textwidth]{pics/motivation_2.png}
% [width=1.30\textwidth]
\caption{Geometrical Structure Consistency can help discriminate samples with noisy correspondence. The retrieval model is first trained on clean Flickr30K dataset, then evaluated on the same dataset with 40\% simulated noise. Left: Calculated cross-modal similarity scores of both clean and noisy samples. Right: Calculated intra-modal similarity scores of both clean and noisy samples. }
\label{Figure: Motivation}
\end{center}
\end{figure}

\subsection{Noise Discrimination \& Purification}

Deep neural networks typically exhibit the memorization effect that tends to initially learn the clean patterns within the dataset before over-fitting on noise. Leveraging this, GSC is able to learn a well-established structure in the early stage, which can be further utilized to predict accurate correspondence indicator.

\noindent
\textbf{Cross-modal Discrimination.} As illustrated in Fig.~\ref{Figure: Structure}(b), based on the well-established cross-modal structure in the early stage, clean data pairs are expected to exhibit more closely aligned cross-modal representations compared to noisy pairs. GSC leverages this structural discrepancy and introduces a function to signify a cross-modal bidirectional correspondence indicator.
\begin{equation}
 y_{\text{CM}}^i = \frac{1}{2}\big[\frac{\exp{(\big<I_i, T_i \big>/\tau_1)}}{\sum_{j}^N\exp{(\big<I_i, T_j\big>/\tau_1)}} + \frac{\exp{(\big<I_i, T_i \big>/\tau_1)}}{\sum_{j}^N\exp{(\big<I_j, T_i\big>/\tau_1})}\big]
\label{Equal: Cross-modal Indicator}
\end{equation}

\begin{figure*}[!t]
\begin{center}
\includegraphics[width=0.8\textwidth]{pics/structure.png}
% [width=1.30\textwidth]
\caption{An overview of GSC. \textbf{Left:} The framework of GSC. GSC simultaneously optimizes both cross-modal and intra-modal objectives to preserve geometrical structure consistency and discriminate samples with noisy correspondence, while the estimated correspondence labels can be further utilized to refine both objective learning. \textbf{Right:} GSC discriminates noisy samples by structural differences from both cross-modal and intra-modal aspects.}
\label{Figure: Structure}
\end{center}
\end{figure*}

\noindent
where $\tau_1$ is the temperature coefficient. For each half of the indicator, it measures the proportion of similarity between the query and the positive key against the similarity between the query and other keys. For a clean sample, the similarity between the query and the positive key should dominate the proportion, thus the value of indicator should approach 1. Conversely, for a noisy sample, the similarity between the query and its positive key would be closer to 0, resulting in the indicator's value trending toward 0.

\noindent
\textbf{Intra-modal Discrimination.} For the intra-modal aspect, the objective function encourages data pairs to exhibit analogous geometrical structures. To illustrate, we compute the similarity vector between a queried image $I_i$ and other images, denoted as $\mathbf{s}_{I_i} =[\big<I_i, I_j\big>]_{j=1}^N$. Similarly, we determine the similarity vector between a queried text $T_i$ and other texts, represented by $\mathbf{s}_{T_i} =[\big<T_i, T_j\big>]_{j=1}^N$. Ideally, matched image-text pairs should have similarity vectors that mirror each other, whereas mismatched pairs would possess distinct similarity vectors, reflecting their divergent positions within a coherent intra-modal structure. Specifically, we employ cosine similarity to measure the resemblance between similarity vectors as follows.
\begin{equation}
 \textbf{s}_{\text{IM}}^i = \frac{\sum_{j=1}^{N} \langle I_i, I_j \rangle \langle T_i, T_j \rangle}{\sqrt{\sum_{j=1}^{N} \langle I_i, I_j \rangle^2} \sqrt{\sum_{j=1}^{N} \langle T_i, T_j \rangle^2}}
 \label{Equal: Cosine Similarity}
\end{equation}

During experiments, the cosine similarity scores of clean samples are observed consistently higher than those of noisy samples, presenting a bimodal distribution of scores across the dataset. This distribution can be accurately modeled using a two-component Gaussian Mixture Model (GMM)~\citep{li2020dividemix}, described by the equation:
\begin{equation}
 p(\textbf{s}_{\text{IM}}) = \sum_{k=1}^K\alpha_k \phi(\textbf{s}_{\text{IM}}|k)
 \label{Equal: GMM}
\end{equation}

Specifically, $\alpha_k$ denotes the $k$-th coefficient and $\phi(\textbf{s}_{\text{IM}}|k)$ is the probability density of the $k$-th component. Consequently, we consider the component with higher values, denoted as $k=k_l$, to represent the estimated score distribution of clean samples. The estimated probability that an observed sample belongs to the clean component $k_l$ can be calculated as follows,
\begin{equation}
 y_{\text{IM}}^i = \frac{\alpha_{k_l}\phi(\textbf{s}_{\text{IM}}^i|k_l)}{\sum_{k=1}^K \alpha_k\phi(\textbf{s}_{\text{IM}}^i|k)}
 \label{Equal: IM indicator}
\end{equation}

So far, we have estimated the true correspondence labels, $y_{\text{CM}}$ and $y_{\text{IM}}$, by leveraging the structural differences in both cross-modal and intra-modal contexts. Our objective is to optimally utilize these two labels to surmount the respective challenges and to accurately identify all samples with noisy correspondence. Therefore, we define the final correspondence label for each sample as the minimum of the two labels, expressed as $y^i = \min\{y_{\text{CM}}^i, y_{\text{IM}}^i\}$.



\input{sec/algo}

\noindent
\textbf{Noise purification.} We address the issue of noisy correspondence by refining both cross-modal and intra-modal objectives. Since the estimated label is a soft label with values in the range of [0, 1] which can directly reflect the degree of true correspondence, we can seamlessly apply it to the loss functions on a sample-wise basis. For the cross-modal objective, we choose the widely-applied contrastive loss as the loss function. The purified cross-modal loss can be denoted as follows,
\begin{equation}
\begin{aligned}
 \mathcal{L}_{\text{CM}} =& -\frac{1}{2N}\sum_{i=1}^Ny^i\log{\frac{\exp{(\big<I_i, T_i\big>/\tau_1)}}{\sum_{j=1}^N\exp{(\big<I_i, T_j\big>/\tau_1)}}} \\
 & -\frac{1}{2N}\sum_{j=1}^Ny^j\log{\frac{\exp{(\big<I_j, T_j\big>/\tau_1)}}{\sum_{i=1}^N\exp{(\big<I_i, T_j\big>/\tau_1)}}}
\label{Equal: Purified Contrastive Loss CM}
\end{aligned}
\end{equation}

For the intra-modal side, in addition to sample-wise purification for the intra-modal loss, it is crucial to prevent the influence of noisy correspondences from distorting the calculation of the geometrical structure. Specifically, when computing the geometrical structure, the distances from the queried sample to those samples with noisy correspondences should be excluded. The purified intra-model loss denotes as, 
\begin{equation}
 \mathcal{L}_{\text{IM}} = -\frac{1}{N}\sum_{i=1}^N\log{\frac{\exp({\sum_{k=1}^N{y^k}^2\big<I_i,I_k\big>\big<T_i,T_k\big>/\tau_2)}}{\sum_{j=1}^N\exp{(\sum_{k=1}^N{y^k}^2\big<I_i, I_k\big>\big<T_j, T_k\big>/\tau_2)}}}
\label{Equal: Purified Contrastive Loss IM}
\end{equation}

Furthermore, noisy correspondences can also interfere with the discrimination of noisy samples during the computation of cosine similarity scores in Eq.~\ref{Equal: Cosine Similarity}. Therefore, a similar modification is employed as follows,
\begin{equation}
 \textbf{s}_{\text{IM}}^i = \frac{\sum_{j=1}^{N} {y^j}^2\langle I_i, I_j \rangle \langle T_i, T_j \rangle}{\sqrt{\sum_{j=1}^{N} (y^j\langle I_i, I_j \rangle)^2} \sqrt{\sum_{j=1}^{N} (y^j\langle T_i, T_j \rangle)^2}}
 \label{Equal: Purified Cosine Similarity}
\end{equation}

The overall loss function of GSC is formulated as a weighted sum of two loss functions, as expressed in the following equation,
\begin{equation}
\label{Equal: Total Loss}
 \mathcal{L} = \mathcal{L}_{\text{CM}} + \gamma\mathcal{L}_{\text{IM}}
\end{equation}

\noindent
where $\gamma$ is the hyper-parameter keeping the balance between two losses, therefore preventing the collapse of the intra-modal structure.

\subsection{Training Schedule}

To integrate the estimation of true correspondence labels with the enhancement of cross-modal retrieval learning, we adopt the temporal ensembling technique, drawing inspiration from \citet{liu2020earlylearning}, to iteratively update the estimated correspondence labels. Specifically, both $y_{\text{CM}}$ and $y_{\text{IM}}$ are updated through a momentum-based combination of the estimates from the current epoch $t$ and the previous epoch $t-1$ before taking minimum as shown below, 
\begin{equation}
\begin{aligned}
 y_{\text{CM}}^i[t] &= \beta_1 y_{\text{CM}}^i[t] + (1-\beta_1) y_{\text{CM}}^i[t-1], \\
 y_{\text{IM}}^i[t] &= \beta_2 y_{\text{IM}}^i[t] + (1-\beta_2) y_{\text{IM}}^i[t-1]
 \label{Equal: Momentum Update}
 \end{aligned}
\end{equation}

\noindent
where $\beta_1$ and $\beta_2$ are separate momentum. The estimation of true correspondence labels can be further improved by utilizing two separate neural networks, where the true correspondence labels for each network are computed from the output of the other network. The ablation in Section~\ref{Section: Experiment} shows that two networks can significantly improve the performance. In conclusion, the overall procedure of our Geometrical Structure Consistency (GSC) method is depicted in the pseudo-algorithm~\ref{Algorithm}.

\subsection{More Discussions}

The improvement of our proposed GSC mainly comes from preserving the geometrical structure consistency and better optimizing strategies, which is compatible with most existing methods. In terms of computational complexity, GSC does not introduce additional computational costs when integrated with a backbone that calculates similarity scores directly from representations, while it necessitates two extra forward passes when the backbone computes similarity scores using a similarity module. This requirement is significantly less demanding compared to MSCN, which involves computations for an additional meta-learning model, or BiCro, which compares each sample against a clean subset. While RINCE shares similar computational cost as GSC, the robust loss function without explicitly exclude noisy samples underperforms at higher noise levels. Furthermore, methods based on NCR framework, \textit{i.e.} NCR, MSCN and BiCro, rely on an inseparable dual-network structure, while GSC is effective with a single model. This attribute makes GSC more adaptable to larger models.



==> sec/6_acknowledgement.tex <==
\section*{Acknowledgement}

This work is supported by the National Key R\&D Program of China (No. 2022ZD0160702),  STCSM (No. 22511106101, No. 22511105700, No. 21DZ1100100), 111 plan (No. BP0719010) and National Natural Science Foundation of China (No. 62306178).
